Bring the Heat: Rapid Trajectory Optimization with Pseudospectral Techniques and the Affine Geometric Heat Flow Equation

Generating optimal trajectories for high-dimensional robotic systems in a time-efficient manner while adhering to constraints is a challenging task. This paper introduces PHLAME, which applies pseudospectral collocation and spatial vector algebra to efficiently solve the Affine Geometric Heat Flow (AGHF) Partial Differential Equation (PDE) for trajectory optimization. Unlike traditional PDE approaches like the Hamilton-Jacobi-Bellman (HJB) PDE, which solve for a function over the entire state space, computing a solution to the AGHF PDE scales more efficiently because its solution is defined over a two-dimensional domain, thereby avoiding the intractability of state-space scaling. To solve the AGHF one usually applies the Method of Lines (MOL), which discretizes one variable of the AGHF PDE, and converts the PDE into a system of ordinary differential equations (ODEs) that are solved using standard time-integration methods. Though powerful, this method requires a fine discretization to generate accurate solutions and requires evaluating the AGHF PDE which is computationally expensive for high-dimensional systems. PHLAME overcomes this deficiency by using a pseudospectral method, which reduces the number of function evaluations required to yield a high accuracy solution thereby allowing it to scale efficiently to high-dimensional robotic systems. To further increase computational speed, this paper presents analytical expressions for the AGHF and its Jacobian, both of which can be computed efficiently using rigid body dynamics algorithms. PHLAME is tested across various dynamical systems, with and without obstacles and compared to a number of state-of-the-art techniques. PHLAME generates trajectories for a 44-dimensional state-space system in $\sim5$ seconds, much faster than current state-of-the-art techniques. A project page is available at https://roahmlab.github.io/PHLAME/

==> sections/symbols.tex <==
\section*{List of Symbols}
\subsection*{Colors}
\begin{itemize}
    \item Purple - reachable set
    \item Red - obstacles
    \item Green - goal configuration
\end{itemize}

\subsection*{General Symbols}
\begin{itemize}
  \item $T$: Some final time. Also length(duration) of a trajectory
  \item $t$: Some time such that $t \in [0,T]$
  \item $I$: Identity matrix
  \item $\textbf{0}$: Vector of zeros\
  \item $L^2$: Set of square integrable functions
\end{itemize}

\subsection*{Dynamics Symbols}
\begin{itemize}
  \item $\x$: Vector of States
  \item $\xd$: Vector of Time Derivatives of States
  \item $\xdd$: Vector of Double Time Derivatives of States
  \item $\q$: Joint positions
  \item $\qd$: Joint velocities
  \item $\uu$: Control inputs
  \item $B$: Control input mapping matrix
  \item $\Hq$: Mass Matrix in terms of $q$
  \item $C(\q, \qd)$: Grouped Coriolis and Gravity term in terms of $q$ and $\qd$
  \item $\Fdx$: Drift dynamics
  \item $\Fx$: Control Matrix
  \item $N$: dimension of $q$. e.g. $\x$ will be of dimension $2N$
  
\end{itemize}

\subsection*{AGHF theory Symbols}
\begin{itemize}
%   \item $\lambda_j$: indeterminants
  \item $X_0$: Vector of Initial States
  \item $X_f$: Vector of Final States
  \item $\Xstar$: set of extremal solutions of AGHF
  \item $\X$: Homotopy defining the evolution of the states of the system
  \item $\Xd$: Time Derivatives of States of homotopy 
  \item $\Xdd$: Double Time Derivatives of States  of homotopy
  \item $\xpone$: First $N$ terms of the state vector
  \item $\xptwo$: Second $N$ terms of the homotopy state vector
  \item $\xdpone$: Derivative of the First $N$ terms of the homotopy state vector
  \item $\xdptwo$: Derivative of the Second $N$ terms of the homotopy state vector
  \item $\xddpone$: Double Derivative of the First $N$ terms of the homotopy state vector
  \item $\xddptwo$: Double Derivative of the Second $N$ terms of the homotopy state vector
  \item $\U$: set of all possible inputs
  \item $L$: Lagrangian
  \item $\A$: Action Functional 
  \item $G(x)$: Riemmanian Metric
  \item $\dxds$: LHS of AGHF PDE
  \item $\ddt \dldxd$: First part of Euler-Lagrange equation
  \item $\dldx$: Second part of Euler-Lagrange equation
  \item $\xstardot$: States corresponding to an extremal solution of AGHF
  \item $\xdstar$: State derivatives corresponding to an extremal solution of AGHF
  \item $u^*$: Input corresponding to the extremal solution
  \item $s$: PDE evolution "time" scale
  \item $\smax$: Final PDE evolution "time"
  \end{itemize}
  
  \newpage
  
  \begin{itemize}
  \item $\Fbar$: Matrix used in \eqref{eqn:G(x)} to build the Riemannian metric
  \item $F_c$: Gram-schmidt based matrix to help Riemannian metric
  \item $k$: Dynamics Penalty term in Riemannian metric
  \item $K$: Large diagonal matrix with $k$'s and 1's 
  \item $\Hdot$: Derivative of Mass Matrix
  \item $\Cdot$: Derivative of Grouped Coriolis and gravity terms
  \item $g(\x)$: Constraint function 
  \item $L_b$: Lagrangian with Barrier function
  \item $\J$: Set of inequality constraints
  \item $j$: Constraint index
  \item $g_j(X)$: $j$-th constraint function 
  % \item $R_j(X)$: $j$-th radius
  % \item $O_j(X)$: $j$-th obstacle center coordinates
  % \item $FK_n(X)$: FK coordinates of the $n$-th joint
  % \item $\tau$: penalty term for the sharpnesss of the barrier
  % \item $g_s(X)$: state constraint function
  % \item $b_s(X)$: state barrier function
  % \item $X_{max}$: maximum state value function
  
\end{itemize}

\subsection*{Pseudospectral Symbols}
\begin{itemize}
  \item $\Omega$: PS AGHF dynamics function
  \item $\frac{\partial \X}{\partial s}$: AGHF LHS
  \item $\FDuzero$: Forward dynamics with $U=0$
  \item $\psX_i(s)$: Solution of the AGHF at the $i$-th chebyshev node at $s$
  \item $\psX(s)$: Vector of solutions to the AGHF at all the chebyshev nodes at $s$
  
  
\end{itemize}

\newpage

